Natural Gradient Hybrid Variational Inference with Application to Deep Mixed Models

Stochastic models with global parameters and latent variables are common, and for which variational inference (VI) is popular. However, existing methods are often either slow or inaccurate in high dimensions. We suggest a fast and accurate VI method for this case that employs a well-defined natural gradient variational optimization that targets the joint posterior of the global parameters and latent variables. It is a hybrid method, where at each step the global parameters are updated using the natural gradient and the latent variables are generated from their conditional posterior. A fast to compute expression for the Tikhonov damped Fisher information matrix is used, along with the re-parameterization trick, to provide a stable natural gradient. We apply the approach to deep mixed models, which are an emerging class of Bayesian neural networks with random output layer coefficients to allow for heterogeneity. A range of simulations show that using the natural gradient is substantially more efficient than using the ordinary gradient, and that the approach is faster and more accurate than two cutting-edge natural gradient VI methods. In a financial application we show that accounting for industry level heterogeneity using the deep mixed model improves the accuracy of asset pricing models. MATLAB code to implement the method can be found at: https://github.com/WeibenZhang07/NG-HVI.

==> acknowl.tex <==

\vspace{0.75em}
\noindent{\large {\bf Acknowledgments}}\\
Nadja Klein gratefully acknowledges funding from the German Alexander von Humboldt foundation. We thank
MutualArt for providing the print price data. 


==> figs.tex <==

\begin{figure}[!thb]
	\caption{Marginals of Different Gaussian Copula Model VAs}
	\begin{center}
		\includegraphics*[scale = 0.7]{figs/densities.eps}
	\end{center}
	Marginal densities $q_i^{\mbox{\tiny SLN2020}}$ (yellow line) and $q_{\lambda_i}$ at~\eqref{eq:EVAmargin} (red line) of optimal VAs
	to two skew normal (SN) target densities (blue line). Both target distributions have 
	the same Pearson skew of 0.8553 and standard deviation $\sigma_{SN}=1$. 
	Panel~(a) plots VA densities when the target mean is $\mu_{SN}=15$, and
	panel~(b) plots VA densities when the target mean is $\mu_{SN}=0$. Also 
	reported are the KL divergences for the optimal approximations.
	\label{fig:KLmargin}
\end{figure}

\begin{figure}[!tb]
	\caption{Kullback-Leibler Divergence of Gaussian Copula Model VA Marginals}
	\begin{center}
		\includegraphics*[scale = 0.8]{figs/Surface.eps}
	\end{center}
	KL divergence of optimal marginal approximations to SN target densities. 
	The SN distributions have a Pearson skew of 0.8553, but different means $\mu_{SN}$ and standard
	deviations $\sigma_{SN}$. Gaussian approximations have KL divergence
	of 0.172 for all target densities (black dashed line), and the approximation $q_{\lambda_i}$ at~\eqref{eq:EVAmargin} has KL divergence of 0.009 for all target densities (solid black line). The KL divergence of $q_i^{\mbox{\tiny SLN2020}}$ is plotted as curves for four values of $\sigma_{SN}$ and $0<\mu_{SN}<60$. 
	The two cases corresponding to Figure~\ref{fig:KLmargin}(a,b) are indicated with circles.
	\label{fig:KLSN}
\end{figure}

\begin{figure}[!tb]
	\caption{Accuracy of Posterior Moments for Mixed Logistic Regression Example}
	\begin{center}
		\includegraphics*[trim = 3cm 1cm 3cm 1cm,clip,width=\textwidth]{figs/Polypharm_moments.eps}
	\end{center}
Panels (a)--(c) are for the t-copula model VA proposed here, and panels~(d)--(f) are for the Gaussian copula model VA in~\cite{smith2020trans}.
In each panel the exact posterior moment (computed using MCMC) is plotted on the horizontal axis, 
and moment of the VA on the vertical axis. The posterior means, standard deviations and Pearson's skew are plotted in the first, second and third columns, respectively. 
In each panel there is a scatter of $m=509$ 
points for each of three variational estimators that correspond to the YJ (blue circles),
iGH (red cross) and YJ-Double (yellow square) transformations for $t_{\gamma_i}$.
For panels~(a)--(e), the results
are very similar for the three transformations, so that most points are close to each other and hard to distinguish.
	\label{fig:polymoments}
\end{figure}

\begin{figure}[!tb]
	\caption{Posteriors for Three Random Effects in the Mixed Logistic Regression Example}
	\begin{center}
		\includegraphics*[trim = 3cm 0cm 3cm 0cm, clip, width=\textwidth]{figs/RE_densities.eps}
	\end{center}
Marginal posterior densities for three random effects.  Each panel plots the exact posterior
computed by MCMC (black line), the t-copula model VA $q_{\lambda_i}$ at~\eqref{eq:qmargin} (red line) and that in~\cite{smith2020trans} $q_i^{\mbox{\tiny SLN2020}}$ (yellow line), both using the iGH transformation. 
	\label{fig:polyRE}
\end{figure}

\begin{figure}[!p]
	\caption{Exact Posterior for the Two U.S. States Inequality Example}
	\begin{center}
		\includegraphics*[width=\textwidth]{figs/CATX_mcmc.eps}
	\end{center}
	Exact posterior of $(\theta_1,\ldots,\theta_5)^\top=(\tau_1,\log \chi_1, \log \nu_1, \log \xi, \log \kappa)^\top$ computed using MCMC. The univariate marginals $p(\theta_i|\yvec)$ are on the leading diagonals, and 
	the bivariate marginals $p(\theta_i,\theta_j|\yvec)$ are on the off-diagonals. 
	\label{fig:CATX_mcmc}
\end{figure}

\begin{figure}[!p]
	\caption{Variational Posterior for the Two U.S. States Inequality Example}
	\begin{center}
		\includegraphics*[width=\textwidth]{figs/CATX_copVA.eps}
	\end{center}
	Posterior estimates of $(\theta_1,\ldots,\theta_5)^\top=(\tau_1,\log \chi_1, \log \nu_1, \log \xi, \log \kappa)^\top$
	using the copula model VA with (adjusted) YJ transformations. 
	The marginals $q_{\lambda_i}(\theta_i)$ are on the leading diagonals, and 
	the bivariate marginals---which are bivariate slices of~\eqref{Eq:VA}---are on the off-diagonals. 
	\label{fig:CATX_copVA}
\end{figure}

\begin{figure}[!tbhp]
	\caption{Variational Posterior Densities of Spearman Correlations for Five Western States}
	\begin{center}
		\includegraphics*[width=0.7\textwidth]{figs/west_spear.eps}
	\end{center}
Variational posterior densities of the 10 Spearman correlations between the contiguous western U.S. states of WA, OR, CA, NV and AZ. The posterior for the
more accurate optimal t-copula is in blue, while that from the mean field t-distribution is in black. 
	\label{fig:west_spear}
\end{figure}


==> sec1_old.tex <==
% !TeX spellcheck = en_US

\section{Introduction}\label{sec:intro}
Black box variational inference (VI) methods~\citep{ranganath2014black} 
that employ a generic
approximating family for the Bayesian posterior distribution are popular.
The approximation is usually learned
by minimizing the
Kullback-Leibler divergence between the two, with 
stochastic gradient ascent\footnote{While it is more common to refer to 
	optimization algorithms as ``descent'', throughout this paper 
	we use the term ``ascent'' instead because our variational optimization is written as a maximization problem.}
	 (SGA) the most common
choice of algorithm to solve the optimization
problem~\citep{bottou10,hoffmanStochasticVariationalInference2013}. Here, the variational approximation (VA)
is updated in the direction of the (noisy) ordinary gradient of the objective function. 
However, the natural gradient gives the steepest direction for this  optimization problem~\citep{amariNaturalGradientWorks1998},
and stochastic natural gradient ascent (SNGA) is an alternative algorithm that
can converge in fewer
steps and avoid plateaus in the objective function~\citep{rattray1998,martensNewInsightsPerspectives2020}. But for large scale problems computing the natural gradient is usually 
impractical for approximations outside the exponential family. 
%For example,
%SNGA is difficult to use when employing rich VAs
%such as normalizing flows~\citep{rezende2015nflow}.
In this paper, we show that the natural gradient can be computed quickly
for the VA family proposed by~\cite{loaiza-mayaFastAccurateVariational2022},
thereby extending the class of VAs to which SNGA can be applied.
Doing so can greatly reduce the time required to learn this approximation
 compared to SGA. 

%We benchmark our approach against existing
%benchmark black box natural gradient methods proposed by~\cite{tranBayesianDeepNet2020} and~\cite{tanAnalyticNaturalGradient2022}, 
%and show that it can be used to learn a heterogeneous Bayesian deep model
%for asset pricing. 
\cite{loaiza-mayaFastAccurateVariational2022} suggested a VI method
where the target vector $\psivec$ is partitioned
into two components $\psivec=(\thetavec^\top,\zvec^\top)^\top$.
The method samples $\zvec$ from its conditional posterior, while using (noisy)
ordinary gradients to update the marginal VA for
% the global model parameters 
$\thetavec$.
%\cite{loaiza-mayaFastAccurateVariational2022} suggested a new 
%approach to undertake VI for the joint
%posterior density of $\psivec=(\thetavec^\top,\zvec^\top)^\top$, where
%$\thetavec$ are
%model parameters and $\zvec$ are latent variables.\footnote{These are also
%called global and local parameters, respectively; for example, see
%\cite{hoffmanStochasticVariationalInference2013}.} 
%The method samples $\zvec$ from its conditional posterior, while using
%re-parameterized stochastic gradients to update the approximation for  $\thetavec$. 
The authors show these two steps together form a
well-defined SGA algorithm
for solving the variational 
optimization for the joint posterior of $\psivec$, and 
%They derive
%re-parameterized gradients~\citep{kingmaAutoEncodingVariationalBayes2014,RezMohWie2014}
%that are fast to compute, 
%and show the approach is both fast and accurate
%for a wide range of problems.
%The authors 
call their method ``hybrid VI''. 
The approach is particularly
attractive when $\zvec$ is a high-dimensional vector of latent variables, which are also sometimes called local
parameters~\citep{hoffmanStochasticVariationalInference2013}.
However, the method can
%The approach is efficient for models with many latent variables, but it 
suffer from slow convergence in common with other first
order stochastic optimization methods for a number of problems, 
such as training some neural networks~\citep{zhangNoisyNaturalGradient2018}. 
In this paper we improve the efficiency of 
hybrid VI by using SNGA optimization. 
The objective is to reduce the number of draws of $\zvec$---typically the slowest step of the algorithm---by 
providing faster convergence of the 
variational optimization. 

The natural gradient 
is equal to the ordinary gradient pre-multiplied by the inverse of the Fisher information matrix (FIM)~\citep{amariNaturalGradientWorks1998}, and the computation, storage and factorization of the latter can be costly.\footnote{While the inverse is not usually computed and stored directly, systems of equations are solved that still require derivation of a factorization of the inverse FIM.} We show that
in hybrid VI the FIM of the VA of $\psivec$
is equal to that of the FIM of the marginal VA of $\thetavec$. 
When 
the dimension of $\thetavec$ is low relative to that of $\zvec$---as is often
the case when $\zvec$ is a vector of latent variables---then 
the additional cost of computing the natural gradient of the VA for $\psivec$ is minor compared to the ordinary gradient.
%
%To evaluate the natural gradient, the main computation is of the inverse Fisher information matrix (FIM).\footnote{While the inverse is not usually computed and stored directly, systems of equations are solved that still require derivation of a factorization of the inverse FIM.} We show that
%the additional cost in computing the natural gradient of the VA for $\psivec$, compared to the ordinary gradient, 
%proves minor in hybrid VI
%because the FIM of the VA of $\psivec$
%is equal to the much lower dimensional FIM of the marginal VA of $\thetavec$. 
This additional cost is more than 
off-set by the savings gained from the smaller number of draws of $\zvec$ required, thus improving the overall efficiency
of the hybrid VI algorithm. 
For the marginal VA of $\thetavec$ we
use a Gaussian distribution with a factor covariance matrix~\citep{miller2017,mishkin2018slang,ongGaussianVariationalApproximation2018,tranBayesianDeepNet2020}. Fast to compute analytical re-parameterized natural gradient updates that use
the Tikhonov damped Fisher information matrix are derived. 
Tikhonov damping,
combined with adaptive learning rates, addresses the
numerical difficulties often encountered with natural gradient
updates when training complex models~\citep{osawa2019large}.

There is growing interest in using NGA in VI. 
\cite{martensNewInsightsPerspectives2020} gives an overview
and discussion of NGA as
a second order optimization method, while
 \cite{martensOptimizingNeuralNetworks2015}, \cite{khanFastSimpleNaturalGradient2018}
 and \cite{zhangFastConvergenceNatural2019} show that  natural gradient based VI methods can improve the efficiency of training neural networks,
 which we also find here.
% by utilizing the information geometry of the approximation density.
\cite{khanFastSimpleNaturalGradient2018} consider the case
where the VA is from the exponential family, and
\cite{linFastSimpleNaturalGradient2019} where the VA 
is a mixture of exponential distributions.
\cite{martensOptimizingNeuralNetworks2015} and~\cite{tranBayesianDeepNet2020} approximate the FIM by block diagonal matrices to reduce computation cost. \cite{tanAnalyticNaturalGradient2022} considers efficient application of SNGA to learn high-dimensional Gaussian VAs based on Cholesky factorization, whereas~\cite{linTractableStructuredNaturalgradient2021} 
suggests transforming the variational parameters to simplify 
 computation of the natural gradient for some fixed form VAs.

We illustrate  our VI approach by using it to estimate several stochastic models. 
Our main focus is on deep mixed models (DMM), which are a class of probabilistic 
Bayesian neural networks. Mixed models (also called random coefficient or multi-level models) are widely used to capture heterogeneity in statistical modeling~\citep{mcculloch2004}, and DMMs extend this approach to deep learning~~\citep{,wikle2019,tranBayesianDeepNet2020,simchoni2021}.
In our DMM  %\citep{bishopPatternRecognitionMachine2006,jospinHandsOnBayesianNeural2022}
the output layer coefficients vary by a group variable and follow a 
 Gaussian distribution, allowing  for heterogeneity. 
 To apply hybrid VI, the vector $\zvec$ contains the output layer group level coefficient values. 
 Using simulation studies, we establish that SNGA is much faster and 
 more reliable than SGA for learning the VA in hybrid VI. We also show 
 for our examples that the natural gradient 
 hybrid VI is faster and more accurate than the alternative 
 natural gradient based VI methods
 of~\cite{tranBayesianDeepNet2020} and~\cite{tanAnalyticNaturalGradient2022}. 
 
%  Using simulated data, we show that SNGA is much faster than SGA for learning the VA in hybrid VI. We also benchmark our proposed approach against the two  recent natural gradient based VI methods proposed by \cite{tranBayesianDeepNet2020} and~\cite{tanAnalyticNaturalGradient2022}. 
%Our method proves both faster and more accurate than these two benchmarks. 

Recent studies suggests that deep models have strong potential in 
financial 
modeling~\citep{guEmpiricalAssetPricing2020,guAutoencoderAssetPricing2021,fangMachineLearningBased2021}.  We use our approach to estimate three factor~\citep{famaCommonRiskFactors1993} and five factor~\citep{famaFivefactorAssetPricing2015} 
financial asset pricing models. We use monthly returns on 2583 stocks between
January 2005 and December 2014 to train a DMM with feed forward neural network architecture that accounts for heterogeneity 
in 548 industry groups. 
Accuracy of the learned model is assessed using posterior predictive distributions computed
for both the training data, and also for a validation period from January 2015 to December 2019. The results suggest that the DMM improves probabilistic 
predictive accuracy
compared to existing (non-deep) linear mixed modeling, and (non-mixed) feed forward neural networks.

%To summarize, our paper makes four contributions. First, we
%evaluate the natural gradient for the VA in hybrid VI, and then show
%that SNGA provides a substantial increase in computational efficiency.
%Second,  we show how to use the natural gradient hybrid VI method to 
%learn DMMs efficiently. Third, 
%
%\noindent\textbf{In summary, our main contributions are:}
%\begin{itemize}
%	\item First, we derive a fast to evaluate natural gradient expression for hybrid variational approximations. The use of the natural gradient leads to a dramatic increase in computational efficiency of hybrid variational inference.
%	\item Second, we demonstrate that when it comes to hybrid variational inference, the use of the natural gradient - as opposed to the stochastic gradient - leads to much faster estimation of deep mixed models with big data sets and large parameter sets.
%	\item Third, we demonstrate in numerical experiments \color{red} and an empirical example (we are not comparing methods in empirical example) \color{black} that hybrid variational inference with natural gradients leads to faster and more accurate estimation of deep mixed models when compared to existing methods such as \cite{tranBayesianDeepNet2020} and \cite{tanAnalyticNaturalGradient2022}.
%	\item Fourth, we apply our method to estimation of a deep mixed model for financial returns. The deep mixed model leads to improvement in asset pricing accuracy, which demonstrates the importance of accounting for heterogeneity and complex fixed effects in financial factor models.
%	
%	
%\end{itemize}


The rest of the paper is organized as follows. Section~\ref{sec:hvi} provides
a brief introduction to the hybrid VI approach, and  Section~\ref{sec:nghvi} extends
hybrid VI to employ the natural gradient. 
Section~\ref{sec:hvidmm} outlines DMMs and in simulation 
studies shows how 
natural gradient hybrid VI leads to an increase in computational efficiency and accuracy for training a DMM,  
compared to both ordinary gradient hybrid VI and the benchmark natural gradient methods
of~\cite{tranBayesianDeepNet2020} and~\cite{tanAnalyticNaturalGradient2022}. 
Section~\ref{sec:finance} contains the financial asset pricing study, while Section~\ref{sec:disc} concludes.

==> sec2_old.tex <==
\section{Hybrid Variational Inference}
This section provides a brief overview of the variational inference and a recently developed hybrid variation approximation family. We then explore the application of different optimization methods using the hybrid variation approximation family. %One of our key contributions to the current literature is that we show that the hybrid variation approximation family can be readily applied to the natural gradient method. With the hybrid approximation method, we can exploit the potential advantage of fast convergence of the natural gradient method with minor additional computational costs compared to the conventional gradient method. At the end of this section, we show the performance of different optimization methods using simulated data.

\subsection{Variational inference for latent variable models}
%Description of the hybrid variational inference, with references to other papers (i.e. literature review) introduce the notation we use. Our hybrid approximation (i.e. define q) here.
We consider Bayesian inference with observed data $\yvec$ and model parameters $\psivec$. Assuming a prior density $p(\psivec)$, Bayesian inference focuses on the posterior density $p(\psivec|\yvec) \propto p(\yvec | \psivec) p(\psivec)$, where $p(\yvec|\psivec)$ is the likelihood of data $\yvec$. In variational inference, the often intractable exact posterior $p(\psivec|\yvec)$ is approximated by a member of more tractable density family $q_{\lambdavec}(\psivec)$, where $\lambdavec \in \mathbf{\calR}^m$ is a vector of variational parameters with dimension $m$. Writing the marginal likelihood as $p(\yvec) = \int_{\psivec} p(\yvec|\psivec)p(\psivec)d\psivec$, the following identity holds regardless of the choice of $q_{\lambdavec}(\psivec)$:
\begin{align}
	log\,p(\yvec) = \int q_{\lambdavec}(\psivec) log \frac{p(\yvec|\psivec)p(\psivec)}{q_{\lambdavec}(\psivec)} d\psivec + \int q_{\lambdavec}(\psivec) log \frac{q_{\lambdavec}(\psivec)}{p(\psivec|\yvec)} \label{marginal_y}
\end{align}
The two integrals in equation (\ref{marginal_y}) are the evidence lower bound (ELBO) and Kullback–Leibler (KL) divergence from the variational approximation $q_{\lambdavec}(\psivec)$ to the exact posterior $p(\psivec|\yvec)$, respectively. Typically, the objective of variational inference is to calibrate variational parameter $\lambdavec$ such that it minimize the KL divergence. While the KL divergence is intractable with unknown posterior density $p(\psivec|\yvec)$, the minimization of the KL divergence is equivalent to the maximization of the ELBO as $log\,p(\yvec)$ is a constant. We can write the ELBO as an expectation with respect to $q_{\lambdavec}(\psivec)$ :
\begin{align}
	\calL(\lambdavec) = E_{q_{\lambdavec}(\psivec)}[log\,g(\psivec) - log\, q_{\lambdavec}(\psivec)] \label{elbo}
\end{align}
where $g(\psivec) = p(\yvec|\psivec) p(\psivec)$. Thus variational inference is reformulated as an stochastic optimization problem and allows easy application of stochastic gradient ascent (SGA) method. \cite{ormerodExplainingVariationalApproximations2010,bleiVariationalInferenceReview2017} provide more detail on variational inference, \cite{zhangAdvancesVariationalInference2019} gives an overview of some recent development in variational inference.\\

Now consider a model with latent variables where the unknown parameter vector $\psivec = (\thetavec^\top,\zvec^\top)^\top$ includes model parameters $\thetavec$ and latent variables $\zvec$. Examples of such model include mixed models where $\zvec$ are realization of random effects \citep{tranBayesianDeepNet2020}, tobit model where $\zvec$ is underlying uncensored data \citep{danaherAdvertisingEffectivenessMultiple2020} and state-space model where $\zvec$ is the latent states \citep{wangStructuredVariationalInference2022}. In the current literature, there are several ways to handle the latent variables $\zvec$. The most straight forward way is to augment the approximation density $q_{\lambdavec}(\psivec)$ to incorporate the latent variables directly \citep{loaiza-mayaVariationalBayesEstimation2019,tanUseModelReparametrization2021,tanAnalyticNaturalGradient2022}. Other researches use a structured variational design to partition all parameters into local and global parameter, and assume independence between VA parameters to reduce the computational costs\cite{hoffmanStructuredStochasticVariational2015}. \cite{tranBayesianDeepNet2020,gunawanFastInferenceIntractable2017} use important sampling to integrate out the latent variables. These methods are either computational costly or introduces extra variances in approximation process and leading to a less accurate approximation. \cite{loaiza-mayaFastAccurateVariational2022} introduces a hybrid method where the latent variables $\zvec$ are sampled from exact conditional posterior using MCMC method and then calibrate other model parameters $\thetavec$ conditional on $\zvec$ using standard optimization method. They approximate the augmented posterior density $p(\psivec|\yvec) = p(\thetavec,\zvec|\yvec) \propto p(\yvec|\thetavec,\zvec)p(\zvec|\thetavec)p(\thetavec)$ with variational approximation of following form
\begin{align}
	q_{\lambdavec}(\psivec) = p(\zvec|\thetavec,\yvec) q^0_{\lambdavec}(\thetavec) 
	\label{hybrid_q}
\end{align}
and show that the gradients required in the optimization steps take the following form
\begin{align}
	\nabla_{\lambdavec} \calL(\lambdavec) = E_{q^0_{\lambdavec}}\left[\frac{\partial \thetavec^\top}{\partial \lambdavec }\left(\nabla_{\thetavec} log \, g(\thetavec,\zvec) - \nabla_{\thetavec} log\,q^0(\thetavec)\right)\right]
	\label{gradient}
\end{align}
where $g(\thetavec,\zvec) = p(\yvec|\thetavec,\zvec)p(\zvec|\thetavec)p(\thetavec)$. With such variational approximation form, the algorithm reduces the approximation error from generate latent variables $\zvec$ as it's generated from exact conditional posterior density. In addition, the optimization step only requires gradients of the ELBO with respect to $\thetavec$, which can potentially greatly reduce the dimension of the gradient by marginalize out $\zvec$ and keep the gradients in a relatively simple form. Readers are referred to \cite{loaiza-mayaFastAccurateVariational2022} for more details of the hybrid method and a review on alternative variation approximations for model with latent variables.
	

\subsection{Stochastic gradient optimization for variational inference}
%step size, reparameterization trick, ?\\
%Stochastic gradient optimization using the re-parameterization technique. Restate the gradient and ELBO results for the hybrid approximation. Extending these to the natural gradient (this is our key methodological contribution).\\

\subsubsection{Stochastic gradient ascent}
In most cases, the ELBO $\calL(\lambdavec)$ is intractable and stochastic gradient ascent (SGA) is a popular method to maximize the ELBO. With an initial value $\lambdavec^{(1)}$, the SGA update $\lambdavec$ recursively as:
\begin{align}
	\lambdavec^{(i+1)} = \lambdavec^{(i)} + \rhovec_i \circ \widehat{\nabla_{\lambdavec} \calL(\lambdavec^{(i)})}
\end{align}
until certain condition is satisfied. Here $\rhovec_i$ is a vector determine the updating size of each element in $\lambdavec$, $\widehat{\nabla_{\lambdavec} \calL(\lambdavec^{(i)})}$ is an unbiased estimates of the gradient of $\calL(\lambdavec)$ with respect to $\lambdavec$ evaluated at $\lambdavec^{(i)}$ and $\circ$ represents element-wise product of two vectors. With appropriate step size $\rhovec_i$ that satisfies the the Robbins-Monro condition \citep{robbinsStochasticApproximationMethod1951}:
\begin{align*}
	\rhovec_i &> 0\\
	\sum_{i = 1}^{\infty}\rhovec_i &= \infty\\
	\sum_{i = 1}^{\infty}\rhovec_i^2 &< \infty
\end{align*}
the algorithm will converge to a local maximum value of $\calL(\lambdavec)$. There are a wide variety of choices for $\rhovec$, for example fixed learning rate \citep{tranBayesianDeepNet2020}, adaptive learning rate \citep{ongVariationalBayesSynthetic2018}, ADADELTA \citep{ongGaussianVariationalApproximation2018} and ADAM \citep{khanFastScalableBayesian2018}. For more about step size go to \cite{mandtVariationalAnalysisStochastic2016}. \\

To complete the updating step, we use the re-parameterization trick to obtain an unbiased estimate ${\nabla_{\lambdavec} \calL(\lambdavec^{(i)})}$. Consider variation approximation of the form in equation (\ref{hybrid_q}). Assume $\epsilonvec = ((\epsilonvec^0)^\top, \zvec^\top)^\top$ have the product density function $f_\epsilon(\epsilonvec) = f_{\epsilon^0}(\epsilonvec^0)p(\zvec|h^0(\epsilonvec^0,\lambdavec),\yvec)$ where $f_{\epsilon^0}(\cdot)$  is a density function that does not depends on $\lambdavec$ and $\thetavec = h^0(\epsilonvec^0,\lambdavec)$. Then the  re-parameterized form of equation (\ref{gradient}) is
\begin{align}
	\nabla_{\lambdavec} \calL(\lambdavec) = E_{f_\epsilon}\left[\frac{\partial \thetavec^\top}{\partial \lambdavec }\left(\nabla_{\thetavec} log \, g(\thetavec,\zvec) - \nabla_{\thetavec} log\,q^0(\thetavec)\right)\right]
	\label{reparameterize_gradient}
\end{align}

Then $\widehat{\nabla_{\lambdavec} \calL(\lambdavec)}$ can be obtained by first generate $\thetavec$ from $h^0(\epsilonvec^0,\lambdavec)$ using a few draws from  $f_{\epsilon^0}(\epsilonvec^0)$, and then generate $\zvec$ from its conditional posterior $p(\zvec|\thetavec,\yvec)$ using a few Gibbs sweeps. Algorithm \ref{fit} outlines the steps to calibrate variational parameters using hybrid methods. Here $R$ is the number of Gibbs sweep for generating $\zvec$. Algorithm \ref{fit} outlines the hybrid SGA method.

\begin{algorithm}[ht!]
	\begin{algorithmic}
		\State Initiate $\lambdavec^{(1)}$ and set $i = 1$
		\Repeat
		\State (a) Generate $\thetavec^{(i)} \sim q_{\lambda^{i}}^0(\thetavec)$ using its re-parametrized representation.
		\For{$r = 1:R$} 
		\State (b)  Generate ${\zvec}^{(i)} \sim p(\zvec| {\thetavec}^{(i)},\yvec)$.
		\EndFor
		\State (c) Compute the gradient $\widehat{\nabla_{\lambda}\mathcal{L}(\lambdavec^{(i)})}$.% or natural gradient $\overline{\nabla_{\lambda}\mathcal{L}(\lambdavec^{(i)})}$.
		\State (d) Compute step size $\boldsymbol{\rho}^{(i)}$.% using the ADADELTA method. 
		\State (e) Set $\lambdavec^{(i+1)} = \lambdavec^{(i)} + \boldsymbol{\rho}^{(i)} \circ \widehat{\nabla_{\lambda}\mathcal{L}(\lambdavec^{(i)})}$.% for the normal gradient method or
		%\State \quad   $\lambdavec^{(i+1)} = \lambdavec^{(i)} + \boldsymbol{\rho}^{(i)} \circ \overline{\nabla_{\lambda}\mathcal{L}(\lambdavec^{(i)})}$ for the natural gradient method.
		\State (f) Set $i = i+1$.
		\Until{the stopping rule is satisfied or a fixed number of steps is completed.}
	\end{algorithmic}
	\caption{Hybrid VI with Stochastic Gradient Optimization}\label{fit}
\end{algorithm}


%\cite{Zhang2019} follows \cite{Hoffman2013} consider models with global parameters and local parameters, where the local parameters are data point specific. They focus on conditional conjugate priors.  \\

% \cite{Hoffman2013} use natural gradient update for models in the conditionally conjugate exponential family. While 
\subsubsection{Natural gradient ascent} 
% natural gradient project the distance of two distributions onto a Riemannian space, where the distance between two distributions is measured by KL divergence, instead of $L_2$ norm as in the regular gradient ascend method. In regular gradient ascend method, the 
While the gradient is widely used in stochastic optimization methods, it does not necessarily represent the steepest direction to reduce the distance between two distributions. Instead, the natural gradient \citep{amariNaturalGradientWorks1998} can potentially improve the efficiency of the optimization by taking into account the information geometry of the objective function. \\

To derive the natural-gradient stochastic optimization, we first need to introduce the Fisher Information Matrix (FIM). The FIM, denoted as $F(\lambdavec)$, is related to the Hessian of KL-divergence between two distributions $q_{\lambda}(\psivec)$ and $q_{\lambda'}(\psivec)$:
\begin{align*}
	KL[q_{\lambda}(\psivec) || q_{\lambda'}(\psivec)] & = E_{q_{\lambda}(\psivec)}[log\, q_{\lambda}(\psivec)] - E_{q_{\lambda}(\psivec)}[log\, q_{\lambda'}(\psivec)]\\
	\nabla_{\lambda'} KL[q_{\lambda}(\psivec) || q_{\lambda'}(\psivec)] & = 	\nabla_{\lambda'} E_{q_{\lambda}(\psivec)}[log\, q_{\lambda}(\psivec)] - 	\nabla_{\lambda'} E_{q_{\lambda}(\psivec)}[log\, q_{\lambda'}(\psivec)]\\
	& = - 	\nabla_{\lambda'} E_{q_{\lambda}(\psivec)}[log\, q_{\lambda'}(\psivec)]\\
	& = - 	 E_{q_{\lambda}(\psivec)}[ \nabla_{\lambda'} log\, q_{\lambda'}(\psivec)]\\
	& = - \int q_{\lambda}(\psivec)  \nabla_{\lambda'} log\, q_{\lambda'}(\psivec) d\psivec\\
	\nabla^2_{\lambda'} KL[q_{\lambda}(\psivec) || q_{\lambda'}(\psivec)] & =  - \int q_{\lambda}(\psivec)  \nabla^2_{\lambda'} log\, q_{\lambda'}(\psivec) d\psivec\\
	& = -  E_{q_{\lambda}(\psivec)}[ \nabla^2_{\lambda'} log\, q_{\lambda'}(\psivec)]\\
	& = - E_{q_{\lambda}(\psivec)}[ H_{log \,q_{\lambda'}(\psivec)}]\\
	& = F_{log \,q_{\lambda'}(\psivec)}
\end{align*}

If we evaluate $F_{log \,q_{\lambda'}(\psivec)}$ at $\lambdavec' = \lambdavec$, then $F = E_{q_{\lambda}(\psivec)}[\nabla_{\lambda} log \,q_{\lambda}(\psivec) \nabla_{\lambda} log \,q_{\lambda}(\psivec)^\top] $ is also the second derivative of $	KL[q_{\lambda}(\psivec) || q_{\lambda'}(\psivec)]$ with respect to $\lambdavec'$, which measures the curvature of the log approximation density.\\

The stochastic gradient can be seen as the result of the following constrained optimization:
\begin{align}
	\lambdavec_{t+1} = \max_{\lambda} \lambdavec^\top \left[ \widehat{\nabla_{\lambda}\calL(\lambdavec_t)}\right] - \frac{1}{2 \alpha_t}(\lambdavec - \lambdavec_t)^\top (\lambdavec - \lambdavec_t)
	\label{lg_sgd}
\end{align}  
which is optimization with distance penalty that prevents the optimization from going too far. In equation (\ref{lg_sgd}) the distance is measured by the $L_2$ norm of the variational parameter.\\

In variational inference, we are optimizing parameters of a distribution to reduce the distance between the fixed form approximation density with the target density. A common measurement of difference between two distribution is KL divergence and we show that the KL divergence can be approximated by a Mahalanobis metrics. The second order Taylor expansion  of $KL[p(\lambdavec_t)||p(\lambdavec_t + d)]$ is:
\begin{align*}
	KL[p(\lambdavec_t)||p(\lambdavec_t + d)] & \approx KL[p(\lambdavec_t)||p(\lambdavec_t )] + (\nabla_{\lambda'}KL[p(\lambdavec_t)||p(\lambdavec_t' )]\mid_{\lambdavec_t' = \lambdavec_t})^\top d + 1/2d^\top F(\lambdavec_t)d
\end{align*}
The first term of the last equation is $0$ by the definition of KL divergence and $\nabla_{\lambda'}KL[p(\lambdavec_t)||p(\lambdavec_t' )]\mid_{\lambdavec_t' = \lambdavec_t} = E_{p(\lambda_t)}[\nabla_{\lambda_t'}log p(\lambdavec_t')] = 0$ using log-derivative trick. So the last equation can be simplified as $[KL[p(\lambdavec_t)||p(\lambdavec_t + d)]  \approx 1/2 d^\top F(\lambdavec_t)d$. Thus we can update the distance measurement in equation (\ref{lg_sgd}) and a revised Lagrangian equation for the natural-gradient descendant step is:
\begin{align}
	\lambdavec_{t+1} = \max_{\lambda} \lambdavec^\top \left[ \widehat{\nabla_{\lambda}\calL(\lambdavec_t)}\right] - \frac{1}{2 \alpha_t}(\lambdavec - \lambdavec_t)^\top F(\lambdavec_t)(\lambdavec - \lambdavec_t)
	\label{lg_ngd}
\end{align}  
and the corresponding update for each step is:
\begin{align}
	\lambdavec_{t+1} = \lambdavec_t + \alpha_t [F(\lambdavec_t)]^{-1}\widehat{\nabla_{\lambda}\calL(\lambdavec_t)}
\end{align}
we will use $\tilde{\nabla} = [F(\lambdavec_t)]^{-1}\widehat{\nabla_{\lambda}\calL(\lambdavec_t)}$ to denote the natural-gradient  as oppose to the standard gradient $\nabla =\widehat{\nabla_{\lambda}\calL(\lambdavec_t)}$. 

\subsection{Natural-Gradient Methods in Hybrid Variational Approximation}
In this section we first prove that the FIM of the hybrid VA is equivalent to the FIM of a simple density. Then we explain techniques to address the computational instability in NGA. Finally we illustrate the advantage of the hybrid natural gradient method using a small simulation study.
\subsubsection{Fisher information matrix of hybrid variation approximation}
Now consider the model where $\psivec = (\thetavec^\top,\zvec^\top)^\top$ and $p(\psivec|\yvec) = p(\thetavec,\zvec|\yvec)\propto p(\yvec|\thetavec,\zvec)p(\zvec|\thetavec)p(\thetavec)$.  Assume the corresponding VAs have the form 
\[q_{\lambda}(\thetavec,\zvec) = p(\zvec|y,\thetavec)q_{\lambda}^0(\thetavec)\]

\cite{loaiza-mayaFastAccurateVariational2022} has shown that the lower bound of the variational approximation 
\begin{align}
	\mathcal{L}(\lambdavec) & = E_{q\lambda}[log\, g(\psivec) - log\, q_{\lambda}(\psivec)]\\
	& =  E_{q\lambda}[log\, g(\thetavec,\zvec) - log\, q_{\lambda}(\thetavec,\zvec)]\\
	& = E_{q\lambda}[log\, p(|\thetavec)  + log\, p(\thetavec)- log\, q^0_{\lambda}(\thetavec)]\\
	& = \mathcal{L}^0(\lambdavec)
\end{align}
where $ \mathcal{L}^0(\lambdavec)$ is the lower bound with $\zvec$ integrated out analytically. The corresponding gradient is
\begin{align}
	\nabla_{\lambda}\mathcal{L}(\lambdavec) = E_{q\lambda}\left[\frac{\partial \thetavec^\top}{\partial \lambdavec}(\nabla_{\theta} log\, g(\thetavec,\zvec) - \nabla_{\theta} log\, q_{\lambda}^0(\thetavec))\right]
\end{align}
To utilise the natural-gradient method with similar convenience, we need to show that the FIM of $q_{\lambda}(\psivec)$ is equivalent to the FIM of $q^0_{\lambda}(\thetavec)$. 

\begin{theorem}[KL equivalence]
	Let the variational approximation density take the form $q_{\lambda}(\thetavec,\zvec) = p(\zvec|y,\thetavec)q_{\lambda}^0(\thetavec)$, then
	\begin{align}
		KL[	q_{\lambda}(\psivec)||q_{\lambda'}(\psivec)]|_{\lambda' = \lambda} = KL[q^0_{\lambda}(\thetavec)||q^0_{\lambda'}(\thetavec)]|_{\lambda' = \lambda
		}
	\end{align} 
\end{theorem}

\begin{proof}
	
	\begin{align*}
		KL[	q_{\lambda}(\psivec)||q_{\lambda'}(\psivec)] & = \int_{\psi} q_{\lambda}(\psivec)[log\,q_{\lambda}(\psivec) - log \,q_{\lambda'}(\psivec)]d(\psivec)\\ 
		& = \int_{\theta} \int_z p(\zvec|y,\thetavec) q^0_{\lambda}(\thetavec)\left[log\,\left(p(\zvec|y,\thetavec) q^0_{\lambda}(\thetavec)\right) - log\, \left( p(\zvec|y,\thetavec) q^0_{\lambda'}(\thetavec)\right) \right]d\zvec d\thetavec\\
		& = \int_{\theta} \int_z p(\zvec|y,\thetavec) q^0_{\lambda}(\thetavec)\left[log\, q^0_{\lambda}(\thetavec) - log\,  q^0_{\lambda'}(\thetavec) \right]d\zvec d\thetavec\\
		& = \int_{\theta}  q^0_{\lambda}(\thetavec)\left[log\, q^0_{\lambda}(\thetavec) - log\,  q^0_{\lambda'}(\thetavec) \right] d\thetavec\\
		& = KL[q^0_{\lambda}(\thetavec)||q^0_{\lambda'}(\thetavec)]
	\end{align*}
\end{proof}

We have shown before that Fisher Information Matrix $F$ of $q_{\lambda}(\psivec)$ is the Hessian of the KL-divergence between $q_{\lambda}(\psivec)$ and $q_{\lambda'}(\psivec)$ evaluated at $\lambdavec' = \lambdavec$. So we have:
\begin{corollary}
	$F(\lambdavec) = \nabla^2_{\lambda'}KL[	q_{\lambda}(\psivec)||q_{\lambda'}(\psivec)] \mid_{\lambda' = \lambda}= F^0(\lambdavec) = \nabla^2_{\lambda'}KL[	q_{\lambda}(\thetavec)||q_{\lambda'}(\thetavec)]\mid_{\lambda' = \lambda}.$ 
\end{corollary}

Using the results above, the natural-gradient of $q_{\lambda}(\psivec)$ also equals that of $q^0_{\lambda}(\thetavec)$:
\begin{align*}
	\tilde{\nabla}_{\lambda} \mathcal{L}(\lambdavec) & = F(\lambdavec)^{-1}\nabla_{\lambda}\mathcal{L} (\lambdavec)\\
	& =  F^{0}(\lambdavec)^{-1}\nabla_{\lambda}\mathcal{L} (\lambdavec)\\
	& =  F^{0}(\lambdavec)^{-1}E_{q\lambda}[\frac{\partial \thetavec^\top}{\partial \lambdavec} (\nabla_{\theta}log\,g(\thetavec,\zvec)- \nabla_{\theta}log\,q^0_{\lambda}(\thetavec))]
\end{align*}
which means we can derive natural-gradient with $\zvec$ integrated out analytically. The advantage of using natural-gradient method with hybrid approximation density is we can avoid storing and inverting high-dimensional matrix $F(\lambdavec)$. Instead, we can rely on a lower dimension matrix $F^0(\lambdavec)$. The inversion of $ F^0(\lambdavec)$ is less burdensome and can avoid complex technique to inverse matrix $F(\lambdavec)$.\\

\cite{ongLikelihoodfreeInferenceHigh2018} have derived the FIM for approximation density with factorized covariance matrix $q_{\lambda}(\thetavec) = \phi(\thetavec; \mu, \Sigma)$, where $\Sigma = BB^\top + D^2$. \cite{tranBayesianDeepNet2020} derived an approximation FIM with block diagonal FIM, which leads to more efficient computation of $F^{-1}$ in high-dimensional case using conjugate gradient linear solver. On the other hand, \cite{khanFastSimpleNaturalGradient2018} and  \cite{linSteinLemmaReparameterization2019} calculate the natural-gradient of exponential family without calculating or inverting $F(\lambdavec)$.

\subsubsection{Tikhonov regularization in natural gradient}
A direct application of natural gradient method can be problematic when the objective function is highly nonlinear, such as those arise in training neural network. When combined with variational approximation the situation is more complicated as the objective function is the KL divergence between the approximation density and unknown ``true'' posterior density. One reason for the failure is that the step size indicated by the natural gradient can be very aggressive in the sense that it moves the variational parameters out of the region where direction of the updating is trust-worthy. The direction of updating suggested by the natural gradient is only appropriate within a small adjacent region around the starting point. When the updated variational parameters lie outside this region, the updated parameters could potentially move away from the optimum value or even cause the whole algorithm to fail.\\

In this paper we use ``Tikhonov regularization'' or Tikhonov damping to modify the updating steps so that after each updating the parameters still lie in a region where updating is accurate. The key idea of the Tikhonov damping method is to add a diagonal damping factor into the Fisher Information Matrix. In our case it is $\hat{\mF} = \mF + \lambda \mI$. As the damping factor $\lambda \rightarrow \infty$, the inverse of $\hat{\mF}$ approximate a faction of $\mI_m$ and the natural gradient method becomes a gradient method, and each step is a fraction of gradients.\\

The addition of the damping factor $\lambda$ is equivalent to adding $\lambda$ to the eigenvalues of matrix $\mF$. This can be shown as follows:
\begin{align*}
	\mF &= \mV \mLambda \mV^\top \\
	\mF &+ \mLambda \mI =  \mV \mLambda \mV^\top + \lambda \mV \mV^\top = \mV(\mLambda + \lambda\mI )\mV^\top\\
	&(\hat{\mF})^{-1} = \mV^\top (\mLambda + \lambda\mI)^{-1}\mV	
\end{align*}
Where $\mV$ is the eigenvectors and $\mLambda$ is a diagonal matrix with corresponding eigenvalues on the diagonal. Thus the effect of the damping factor is shrinking the movement of variational parameters by a factor of $\frac{\lambda_j}{\lambda + \lambda_j}$ with $\lambda_j$ being the $jth$ eigenvalue. From this we can see that the parameters with very small $\lambda_j$ will need larger damping factor to avoid large and untrustworthy updates. In practice, if the parameters are operating in similar scales then a single damping factor could work well. However, in the cases where the parameters are in relatively different scales, using an universal damping factor can be inefficient. To account for the scale differences, we adopt the a diagonal damping matrix suggested by \cite{martensTrainingDeepRecurrent2012}, where the damping matrix is the diagonal elements of the original Fisher Information Matrix:
\[\hat{\mF} = {\mF} + \lambda diag({\mF})\]
The intuition is that the elements with larger scale with be assigned a larger damping factor and the smaller elements with be assigned a smaller damping factor. \\

Algorithm \ref{fit_nga} outlines our proposed hybrid NGA method. The optimization process is similar with the SGA method except that in step (c) we update the variational parameters using our proposed stabilized natural gradient.
\begin{algorithm}[ht!]
	\begin{algorithmic}
		\State Initiate $\lambdavec^{(1)}$ and set $i = 1$
		\Repeat
		\State (a) Generate $\thetavec^{(i)} \sim q_{\lambda^{i}}^0(\thetavec)$ using its re-parametrized representation.
		\For{$r = 1:R$} 
		\State (b)  Generate ${\zvec}^{(i)} \sim p(\zvec| {\thetavec}^{(i)},\yvec)$.
		\EndFor
		\State (c) Compute the stabilized natural gradient $\overline{\nabla_{\lambda}\mathcal{L}(\lambdavec^{(i)})} = (\widehat{\mF}^{(i)})^{-1}\widehat{\nabla_{\lambda}\mathcal{L}(\lambdavec^{(i)})}$.% or natural gradient $\overline{\nabla_{\lambda}\mathcal{L}(\lambdavec^{(i)})}$.
		\State (d) Compute step size $\boldsymbol{\rho}^{(i)}$.% using the ADADELTA method. 
		\State (e) Set $\lambdavec^{(i+1)} = \lambdavec^{(i)} + \boldsymbol{\rho}^{(i)} \circ \overline{\nabla_{\lambda}\mathcal{L}(\lambdavec^{(i)})}$.% for the normal gradient method or
		%\State \quad   $\lambdavec^{(i+1)} = \lambdavec^{(i)} + \boldsymbol{\rho}^{(i)} \circ \overline{\nabla_{\lambda}\mathcal{L}(\lambdavec^{(i)})}$ for the natural gradient method.
		\State (f) Set $i = i+1$.
		\Until{the stopping rule is satisfied or a fixed number of steps is completed.}
	\end{algorithmic}
	\caption{Hybrid VI with Stabilized Natural Gradient Optimization}\label{fit_nga}
\end{algorithm}

\subsubsection{Natural-Gradient Methods in Probit Model}
In this section, we conduct a small simulation study to show the improvement of optimization efficiency using NGA method. Consider a probit model with random effect:
\begin{align}
	y_{i,h}^* &= \betavec^\top \xvec_{i,h} + u_h + e_{i,h} \\
	y_{i,h} & = I(y_{i,h}^* > 0)
	\label{latent equation}
\end{align}
where $u_{i}$ represents an additive scalar random effect for individual $i$. Denote $\yvec^{*} = (y_1^*,y_2^*,\dots, y_n^*)^\top,\uvec = (u_{1}, u_{2}, \dots, u_{H})^\top $, $\zvec = (\yvec^{*\top},\uvec^\top)^\top$, and let $\thetavec$ includes all model parameters including $\betavec$. The data simulation process is as follows:
\begin{enumerate}
	\item Set total number of observation n = 2000, number of covariates m = 3. Generate random 3 by 2000 random matrix $\xvec_i \sim N(\muvec_x, \mSigma_x)$ with $\muvec_x = \mathbf{0}_3, \mSigma_x = \mL\mL' + diag(\dvec)$.
	\item Generate $\betavec \sim N(\mathbf{0}_4, 10\mI_4)$. 
	\item Suppose there are 20 individuals in each group, such that $n_h = 20$ for $h = 1, \dots, 20$. Then we have 100 different random effects. Generate $u_h \sim N (0,1)$ for $h = 1, \dots, 100$. 
	\item Generate $e_{i,h} \sim N(0,1)$ for $i = 1, \dots, 20$ and $h = 1, \dots, 100$. 
	\item Generate $y_{i,h}^* = \betavec^\top \xvec_{i,h} + u_h + e_{i,h}$ and $y_{i,h} = I(y_{i,h}^* > 0)$.
\end{enumerate}
In this simulation exercise, we know the real value of latent variable $\yvec^*$ from the data generating process. So we illustrate the convergence of the two algorithms by measuring the root mean squared error (RMSE):
\begin{align}
	RMSE = \sqrt{\frac{\sum_{h = 1}^{100}\sum_{i = 1}^{20}(\hat{y}_{i,h}^* - y_{i,h}^*)^2}{2000}}
\end{align}
where $\hat{y}_{i,h}^*$ is the predicted value from the VI processes and ${y}_{i,h}^*$ is the value from the data simulation. We can see from figure \ref{converge_rmse}, natural-gradient method (NGA) method takes less steps to reach the optimum compared to the stochastic gradient method (SGA). Even though the NGA method requires longer computational time for each step, the NGA method still requires less time to reach the minimum RMSE value.
\begin{figure}[ht!]
	\begin{subfigure}{0.5\linewidth}
		\includegraphics[width=1\linewidth]{Graphs/RMSE_step.pdf}
		\subcaption{Convergence of RMSE against steps}
	\end{subfigure}
	\begin{subfigure}{0.5\linewidth}
		\includegraphics[width=1\linewidth]{Graphs/RMSE_time.pdf}
		\subcaption{Convergence of RMSE against wall clock}
	\end{subfigure}
	\caption{Convergence of RMSE.}
	\label{converge_rmse}
\end{figure}

\subsubsection{Natural-gradient} 
In this section we compare our proposed hybrid NGA method with another natural-gradient method proposed by \cite{tanAnalyticNaturalGradient2022}. For simplicity here we consider a linear mixed model with additive scalar random effect $\alpha_h$. For $h = 1, \dots, H$ :
\begin{align}
	y_{i,h} = \betavec^\top \xvec_{i,h}+ \alpha_h + \varepsilon_{i,h}
\end{align}
here $\betavec$ is a $m \times 1$ vector representing fixed effect, $\xvec_{i,h}$ is a $m\times1$ covariates (predictors) vector. We further assume that $\alpha_h|\sigma^2_\alpha \sim N(0,\sigma^2_\alpha)$ and $\varepsilon_{i,h} \sim N(0,\sigma^2_e)$ for for $h = 1,\dots, H$ and $i = 1, \dots, n$. The parameter space is $\psivec = [\betavec^\top , log(\sigma^2_\alpha), log(\sigma^2_e), \alpha_1, \dots, \alpha_H]^\top$, here we transform the positive parameter $\sigma^2_\alpha$ and $\sigma^2_e$ into real line using log function. \\

For the simulation study we use $m = 6$(including intercept term), $H = 1000$ and the number of observations $n_h=5$ for all groups, thus $\yvec_h$ is a $5\times 1$ vector and $\mX_h$ is a $5\times 6$ matrix for $h = 1,\dots, H$. We use the convergence of ELBO to evaluate the convergence of algorithms and a higher ELBO represents better approximation. \\

\cite{tanAnalyticNaturalGradient2022} approximate the random effects with Gaussian approximation with sparse covariance matrix, which can be restrictive. First this approximation impose the assumption that the posterior of the random effect is also Gaussian, which is not necessarily true. The second is that the sparsity covariance matrix of random effect impose independent assumption between local parameters and global parameters. Even with re-parameterization method proposed by \cite{tanUseModelReparametrization2021} to  mitigate the restriction, this can lead to inaccurate posterior for random effects. Lastly, this approximation can introduce more noise to the overall calibration of variational parameters, and can be costly when the dimension of local parameters is large.\\

Figure \ref{ELBO_LMM_tan} compare the convergence of ELBO using different methods. Here the true DGP has moderate variation for both error term and random effect, so that $\sigma^2_e = \sigma^2_\alpha = 1$, and use $1$ factor for the factorized covariance matrix in our hybrid NGA method. \\

\begin{figure}[ht!]
	\begin{subfigure}{0.5\linewidth}
		\includegraphics[width=1\linewidth]{Graphs/compare_ELBO_LMM_sigma_a_1_P_1.pdf}
		\subcaption{Convergence of ELBO against step.}
	\end{subfigure}
	\begin{subfigure}{0.5\linewidth}
		\includegraphics[width=1\linewidth]{Graphs/compare_time_ELBO_LMM_sigma_a_1_P_1.pdf}
		\subcaption{Convergence of ELBO against clock-time.}
	\end{subfigure}
	\caption{Comparison of convergence of ELBO between DAVI and hybrid NGA.}
	\label{ELBO_LMM_tan}
\end{figure}
As the Gibbs sampling is also feasible in this simulation study, we also compare the results of two VIs with the Gibbs samplings. Figure (\ref{MCMC_LMM_tan}) shows the posterior of model parameters using three different methods. The approximated posteriors of our proposed hybrid method are very close to the results of MCMC for both $\betavec$, error variance $\sigma^2_e$ and random effect variance $\sigma^2_\alpha$. On the other hand, Tan's method tends to underestimate the variance of posterior densities for some model parameters. Most importantly, Tan's method fails to correctly calibrate the variance of random effect, resulting a shift of approximation density for $log(\sigma^2_\alpha)$, which may also leads to the mis-calibrated intercept term. 
\begin{figure}[ht!]
	\centering
\begin{subfigure}{0.8\linewidth}
	\includegraphics[width=1\linewidth]{Graphs/LMM_sigma_a_1posterior_beta.pdf}
	\subcaption{posterior of $\betavec$}
\end{subfigure}

\begin{subfigure}{0.45\linewidth}
	\includegraphics[width=1\linewidth]{Graphs/LMM_sigma_a_1posterior_sigma2_e.pdf}
	\subcaption{posterior of $log(\sigma^2_e)$}
\end{subfigure}
\begin{subfigure}{0.45\linewidth}
	\includegraphics[width=1\linewidth]{Graphs/LMM_sigma_a_1posterior_sigma2_a.pdf}
	\subcaption{posterior of $log(\sigma^2_\alpha)$}
\end{subfigure}
\caption{Comparison of posterior density. The MCMC method runs for 1000 steps and drop first 500 steps as burn-in.}
\label{MCMC_LMM_tan}
\end{figure}

We have done more simulation studies with different combination of variation in error term and random effect, as well as different number of factors for covariance matrix in the hybrid method. The results are stable and our proposed method shows consistent better convergence in terms of ELBO. Table \ref{summary_elbo} summaries the results of different simulation set-ups. %The results of more simulation are available in the appendix \colorbox{red}{HAVE NOT ADD TO THE APPENDIX, need to regenerate the figures}.\\
\begin{table}
	\centering
		\caption{Summary of different simulation set-ups}
\begin{tabular}[ht!]{llcccc}
		\toprule
	&& $p =1 $ &  $p=2$ &  $p=3$& Tan\\
\hline
	\multirow{4}{*}{m = 5, n = 10000, H =100}&$\sigma^2_\alpha = 0.01$ & -7320.0 & -7319.9 & -7319.8 &-7488.9\\
	
	&$\sigma^2_\alpha = 1$ & -7466.7 & -7466.3 & -7466.1 &-7536.0\\
	
	&$\sigma^2_\alpha = 5$ & -7547.1 & -7547.1 & -7547.0&-7664.9\\
	&$\sigma^2_\alpha = 10$ & -7582.2 & -7582.5 & -7582.4&-7759.8\\
	\hline
	\multirow{4}{*}{m = 5, n = 10000, H =10}&$\sigma^2_\alpha = 0.01$ & -7153.1 & -7152.6 & -7151.9 &-11434\\
	
	&$\sigma^2_\alpha = 1$ & -7166.2 & -7164.5 & -7162.4& -11438\\
	
	&$\sigma^2_\alpha = 5$ & -7175.8 & -7172.5 & -7171.8&-11457\\
	&$\sigma^2_\alpha = 10$ & -7179.5 & -7176.2 & -7176.2&-11481\\
	\hline
	\multirow{4}{*}{m = 15, n = 10000, H =10}&$\sigma^2_\alpha = 0.01$ & -7178.2 & -7175.5 & -7175.2 &-13861\\
	
	&$\sigma^2_\alpha = 1$ & -7181.3 & -7179.8 & -7180.3&-13862 \\
	
	&$\sigma^2_\alpha = 5$ & -7187.7 & -7187.1 & -7187.9&-13867\\
	&$\sigma^2_\alpha = 10$ & -7191.6 & -7191.2 & -7191.8&-13873\\
	\bottomrule
\end{tabular}
	\label{summary_elbo}
\end{table}
%\subsection{Comparison of optimization methods} 
%Motivate the computational advantage of NGA and its potential for increasing the speed of convergence at minor computational cost for the hybrid methods. Demonstrate using the probit example. 
\clearpage

==> sec5_old.tex <==
\section{Discussion}\label{sec:disc}
While natural gradient stochastic optimization methods have strong potential in 
variational inference, their use is limited due to the computational
complexity for VAs outside the exponential family.  
In this paper, we propose a natural gradient method (NG-HVI) that employs the VA at~\eqref{eq:hybrid_q}. Doing so has three advantages which we list here.
First,  Theorem~\ref{thm:FIM} and Corollary~\ref{cor:ng} show that the computational complexity of evaluating the natural gradient grows only with 
$\mbox{dim}(\thetavec)$, not the dimension of the target 
density $p(\psivec|\yvec)$. When $\mbox{dim}(\thetavec)<<\mbox{dim}(\psivec)$ (for example, as is the case with many 
latent variable models) this reduces the computational complexity of evaluating 
the natural gradient greatly.  Second, the proposed VA may be far from Gaussian 
because the conditional posterior 
$p(\zvec|\thetavec,\yvec)$ may be also. This density, nor
its derivatives, are not required to implement 
Algorithm~\ref{alg:nghvi}. Instead, it is only necessary to draw from this conditional posterior,
which can be achieved using a wide array of existing methods. 
Last, that approximation at~\eqref{eq:hybrid_q} is necessarily more
accurate than any other VA for $\psivec$ that shares the same marginal $q^0(\thetavec)$.
In practice, the importance of this feature grows with the dimension of $\zvec$, because
the cumulative error of even well-calibrated fixed form VAs for $\zvec$ grows as well.


%\textcolor{red}{Natural gradient based stochastic gradient methods are increasingly used in variational inferences. However, the application of natural gradient method has been restricted due to its computational complexity. In this paper, we proposed an efficient natural gradient method (NG-HVI) that combine the novel hybrid VA proposed in \cite{loaiza-mayaFastAccurateVariational2022} with standard natural gradient method. NG-HVI method addresses some of the roadblocks of using natural-gradient based method for calibration of VA of the form $q_\lambda(\psivec)$, where $\psivec$ consists of global parameter $\thetavec$ and potentially large dimensional latent variable $\zvec$.} In this paper we show how to apply SNGA to learn
%the VA at~\eqref{eq:hybrid_q}, and
%the resulting VI method has a number of advantages that we list here.
%First, for high-dimensional targets $\psivec$,  NGA methods are currently  used with only a limited range of VAs because computation of the 
%natural gradient is costly. 
%In contrast, following
%Theorem~\ref{thm:FIM}, the computation of the FIM and  natural gradient  are unaffected by 
%the dimension of $\zvec$, so that it can be  high.
%Second, the proposed VA may be far from Gaussian
%because the conditional posterior 
%$p(\zvec|\thetavec,\yvec)$ may be also. This density, nor
%its derivatives, are not required to implement 
%Algorithm~\ref{alg:nghvi}. Instead, it is only necessary to draw from this conditional posterior,
%which can be achieved using a wide array of existing methods. 

We demonstrate these advantages in our empirical work. The results suggest
that learning the
VA using SNGA proves  more efficient and stable than using SGA as originally 
suggested by~\cite{loaiza-mayaFastAccurateVariational2022}. The proposed
method also out-performed the two natural gradient benchmark methods for 
our examples. While these examples are latent variable models, NG-HVI can
also be used with 
other stochastic models with $\psivec$  partitioned in other ways, as long as generation of $\zvec$
from its conditional posterior is
viable. For example, $\zvec$ may contain discrete-valued 
parameters, which is a case that is difficult to deal with using standard VI methods~\citep{tran2019discrete}.

Heterogeneity is documented in many studies
and using random coefficients is a popular way of
capturing this~\citep{gelman2006}.
Thus, the DMMs proposed by~\cite{tranBayesianDeepNet2020} that employ 
random coefficients on the output layer of a probabilistic Bayesian 
neural network have strong potential. 
However, DMMs are hard to train because
the posterior is complex and
the dimension of $\zvec$ is often high. Our empirical work demonstrates
that NG-HVI is an effective approach for doing so, and that it improves substantially on SG-HVI.
One alternative is to use importance sampling to integrate out the random 
coefficients, as suggested in the 
original study of~\cite{tranBayesianDeepNet2020}. However, this is more computationally 
demanding than NG-HVI, and the method scales poorly with the number of
output layer nodes. The potential of DMMs is demonstrated in
the financial study, where
the combination of a feed forward neural network and industry-based
heterogeneity produces a significant
increase in predictive accuracy using the Fama and French factors as inputs. 

We finish by noting two directions for further work. First, while we employ
the Gaussian factor covariance VA for $q^0$, 
other VAs for which fast natural gradient updates can be computed 
may also be used. This includes a Gaussian VA
with fast Cholesky updates as suggested by \cite{tanAnalyticNaturalGradient2022},
the 
implicit copula VAs of~\cite{han2016,smithHighDimensionalCopulaVariational2020}, the 
mixture VAs of~\cite{linFastSimpleNaturalGradient2019} or the tractable
fixed forms 
suggested by~\cite{linTractableStructuredNaturalgradient2021}. 
Second, the promising results of the financial study encourage the further exploration of the 
use of DMMs in asset pricing. %Such a study would contribute to evidence that incorporating both heterogeneity and non-linearity in traditional financial models can improve results~\citep{guEmpiricalAssetPricing2020}.


==> tabs.tex <==
\begin{table}[htb]
	\begin{center}
	\small%\renewcommand\arraystretch{1.15}
	\caption{Point forecast accuracy of models during the evaluation period}\label{tab:pointfore}
	\begin{tabular}{llllllll}
		\hline
		&\multicolumn{7}{c}{Hours Ahead in the Forecast Horizon}\\ \cline{2-8}
		Model & 0.5 hour & 1 hour & 2 hours & 3 hours & 6 hours & 12 hours & 24 hours \\ 
		\hline
		&\multicolumn{7}{l}{MAE}\\ \cline{2-8}
GAMLSS & 0.0226$^{***}$ & 0.0314$^{***}$ & 0.0408$^{***}$ & 0.0468$^{***}$ & 0.0591$^{***}$ & 0.0692$^{***}$ & 0.0766$^{***}$ \\ 
  RNN & 0.0249$^{***}$ & 0.0319$^{***}$ & 0.0411$^{***}$ & 0.0494$^{***}$ & 0.0600$^{***}$ & 0.0722$^{***}$ & 0.0800$^{***}$ \\ 
  RNNSN & 0.0221$^{***}$ & 0.0219$^{*}$ & 0.0239 & 0.0252 & 0.0262 & 0.0268$^{**}$ & 0.0278$^{***}$ \\ 
  RNNST & 0.0189 & 0.0210 & 0.0231 & 0.0242 & 0.0250 & 0.0255$^{***}$ & 0.0257$^{***}$ \\ 
 \emph{RNNC}& \emph{0.0169} & \emph{0.0194} & \emph{0.0224} & \emph{0.0238} & \emph{0.0252} & \emph{0.0244} & \emph{0.0239} \\ 
 
		&\multicolumn{7}{l}{RMSE}\\ \cline{2-8}
GAMLSS & 0.0340$^{\mbox{\tiny{+}}}$ & 0.0461$^{\mbox{\tiny{++}}}$ & 0.0610$^{\mbox{\tiny{+++}}}$ & 0.0623$^{\mbox{\tiny{+++}}}$ & 0.0644$^{\mbox{\tiny{+++}}}$ & 0.0653 & 0.0661 \\ 
  RNN & 0.0537 & 0.0616$^{\mbox{\tiny{**}}}$ & 0.0712 & 0.0797 & 0.0935 & 3.7173$^{***}$  & 16.5496$^{***}$  \\ 
  RNNSN & 0.0538 & 0.0572 & 0.0603 & 0.0615 & 0.0623 & 0.0629 & 0.0638 \\ 
  RNNST & 0.0528$^{\mbox{\tiny{+}}}$ & 0.0571 & 0.0603 & 0.0612 & 0.0623 & 0.0630 & 0.0635 \\ 
  \emph{RNNC} & \emph{0.0538 }& \emph{0.0573 }&\emph{ 0.0613} & \emph{0.0638} & \emph{0.0657} & \emph{0.0632} & \emph{0.0629} \\ 
  
%GAMLSS & 0.0455 & 0.0485 & 0.0494 & 0.0480 & 0.0471 & 0.0475 \\ 
%  RNN & 0.0503$^{\mbox{\tiny{+++}}}$ & 0.0507 & 0.0511 & 0.0520 & 0.0535 & 0.0565 \\ 
%  RNNSN & 0.0491 & 0.0485 & 0.0494 & 0.0482 & 0.0492 & 0.0489 \\ 
%  RNNST & 0.0478 & 0.0473 & 0.0474 & 0.0471 & 0.0471 & 0.0474 \\ 
%  {\em RNNC} & {\em 0.0529} & {\em 0.0547} & {\em 0.0542} & {\em 0.0567} & {\em 0.0511} & {\em 0.0486} \\ 
		\hline
	\end{tabular}
\end{center}
		Both the system-weighted mean absolute error (MAE) and root
		mean squared error (RMSE) are reported. Results are given for the four deep time series models, plus GAMLSS. Results of a two-sided Diebold-Mariano test of the equality of the mean error of the RNNC with each of the other models are reported. Rejection of the null hypothesis of equal means at the 10\%, 5\% and 1\% levels are denoted by ``*'', ``**'' and ``***'' if favorable to the RNNC model, or by ``${\mbox{\tiny{+}}}$'', ``${\mbox{\tiny{++}}}$'' and
		``${\mbox{\tiny{+++}}}$'' if unfavorable.
\end{table}

\begin{table}[ht]
\begin{center}
\caption{Probabilistic forecast accuracy during the evaluation period.}\label{tab:densityfore}
\centering\small%\renewcommand\arraystretch{1.25}
\begin{tabular}{lllllllll}
  \hline
		&\multicolumn{7}{c}{Hours Ahead in the Forecast Horizon}\\ \cline{2-8}
		Model & 0.5 hour & 1 hour & 2 hours & 3 hours & 6 hours & 12 hours & 24 hours  \\ \hline
  &\multicolumn{7}{l}{{\em CRPS}}\\ \cline{2-8}
GAMLSS & 0.0180$^{***}$ & 0.0252$^{***}$ & 0.0335$^{***}$ & 0.0392$^{***}$ & 0.0508$^{***}$ & 0.0601$^{***}$ & 0.0652$^{***}$ \\ 
  RNN & 0.0203$^{***}$ & 0.0235$^{***}$ & 0.0299$^{***}$ & 0.0364$^{***}$ & 0.0449$^{***}$ & 0.0574$^{***}$ & 0.4061$^{***}$ \\ 
  RNNSN & 0.0174$^{***}$ & 0.0177$^{**}$ & 0.0191 & 0.0201 & 0.0207 & 0.0212$^{**}$ & 0.0219$^{***}$ \\ 
  RNNST & 0.0157$^{***}$ & 0.0172$^{***}$ & 0.0187$^{***}$ & 0.0195 & 0.0201 & 0.0206$^{***}$ & 0.0208$^{***}$ \\
 \emph{RNNC} & \emph{0.0135} & \emph{0.0154} & \emph{0.0177} & \emph{0.0189} & \emph{0.0199} & \emph{0.0193} & \emph{0.0187} \\ 
  &\multicolumn{6}{l}{{\em Joint Upper Tail Loss at }$\alpha=0.975$}\\ \cline{2-8}
GAMLSS & 31.6394$^{*}$ & 32.4717$^{***}$ & 33.2367$^{***}$ & 33.9396$^{***}$ & 35.9352$^{***}$ & 40.0541$^{***}$ & 39.7960$^{***}$ \\ 
  RNN & 30.8568 & 31.5025 & 33.3171 & 35.5605 & 39.2732$^{**}$ & 41.9374$^{***}$ & 33.4037$^{***}$ \\ 
  RNNSN & 32.1052$^{**}$ & 31.2797 & 31.6342 & 31.6492 & 31.7099 & 31.5852$^{***}$ & 31.3780$^{***}$ \\ 
  RNNST & 31.3493$^{*}$ & 31.4414 & 31.6911 & 32.0056$^{*}$ & 31.8607 & 32.2372$^{***}$ & 31.8694$^{***}$ \\ 
  \emph{RNNC} & \emph{30.1002} & \emph{30.6244} & \emph{31.0090} & \emph{31.0934} & \emph{31.1121} & \emph{30.6238} & \emph{29.7661} \\ 
  
&\multicolumn{7}{l}{{\em Quantile Score at} $\alpha=0.95$}\\ \cline{2-8}
GAMLSS & 0.0056$^{***}$ & 0.0069$^{***}$ & 0.0082$^{***}$ & 0.0093$^{***}$ & 0.0124$^{***}$ & 0.0190$^{***}$ & 0.0198$^{***}$ \\ 
  RNN & 0.0050 & 0.0057 & 0.0078$^{***}$ & 0.0107$^{***}$ & 0.0155$^{***}$ & 0.0201$^{***}$ & 1.0808$^{***}$ \\ 
  RNNSN & 0.0056 & 0.0050 & 0.0054 & 0.0055 & 0.0057 & 0.0058$^{*}$ & 0.0060$^{***}$ \\ 
  RNNST & 0.0048 & 0.0050 & 0.0054 & 0.0057$^{**}$ & 0.0057$^{*}$ & 0.0062$^{***}$ & 0.0063$^{***}$ \\ 
  \emph{RNNC} & \emph{0.0036} & \emph{0.0043} & \emph{0.0048} & \emph{0.0050} & \emph{0.0052} & \emph{0.0050} & \emph{0.0046} \\ 
  
 &\multicolumn{7}{l}{{\em Quantile Score at} $\alpha=0.05$}\\ \cline{2-8}
 
GAMLSS & 0.0049$^{***}$ & 0.0080$^{***}$ & 0.0129$^{***}$ & 0.0167$^{***}$ & 0.0242$^{***}$ & 0.0260$^{***}$ & 0.0298$^{***}$ \\ 
  RNN & 0.0047 & 0.0053 & 0.0057$^{***}$ & 0.0061 & 0.0069$^{***}$ & 0.0096$^{***}$ & 0.5602$^{***}$ \\ 
  RNNSN & 0.0046$^{**}$ & 0.0055 & 0.0056 & 0.0062 & 0.0061 & 0.0064 & 0.0065 \\ 
  RNNST & 0.0048$^{***}$ & 0.0055$^{*}$ & 0.0059$^{**}$ & 0.0061 & 0.0064 & 0.0063 & 0.0066 \\ 
  \emph{RNNC} & \emph{0.0039} & \emph{0.0046} & \emph{0.0053} & \emph{0.0058} & \emph{0.0061} & \emph{0.0059} & \emph{0.0057} \\  
  \hline
\end{tabular}
\end{center}
System-weighted metrics are reported for the four deep time series models, plus
GAMLSS, at different points in time during a 24 hour forecast horizon. 
Lower values suggest greater accuracy. Results of a two-sided Diebold-Mariano test of the equality of the mean error of the RNNC with each of the other models are reported.
Rejection of the null hypothesis of equal means at the 10\%, 5\% and 1\% levels are denoted by ``*'', ``**'' and ``***'' if favorable to the RNNC model, or by ``${\mbox{\tiny{+}}}$'', ``${\mbox{\tiny{++}}}$'' and
``${\mbox{\tiny{+++}}}$'' if unfavorable.
\end{table}

%
%\begin{table}[ht]
%\centering\small\renewcommand\arraystretch{1.25}
%\begin{tabular}{c|cccccc}
%  \hline
%Method & 1 hour & 2 hours & 3 hours & 6 hours & 12 hours & 24 hours \\ 
%  \hline
%RNNC & 0.0472 & 0.0489 & 0.0495 & 0.0525 & 0.0476 & 0.0450 \\ 
%  GAMLSS & 0.0527 & 0.1123 & 0.1013 & 0.1015 & 0.1428 & 0.1975 \\ 
%  RNNST & 0.0419 & 0.0421 & 0.0427 & 0.0429 & 0.0428 & 0.0431 \\ 
%  RNNSN & 0.0440 & 0.0437 & 0.0453 & 0.0441 & 0.0451 & 0.0452 \\ 
%  RNN & 0.0440 & 0.0450 & 0.0457 & 0.0468 & 0.0480 & 0.0504 \\ 
%   \hline
%\end{tabular}
% \caption{System weighted RMSE values computed from the simulated ahead forecast values.
% 	Results from all three models are shown, these are RNNC, GAMLSS, RNNSN, RNN. Lower values correspond to higher predictive accuracy. The system weights are: NSW: 0.3687
%VIC: 0.2355
%QLD: 0.2818
%TAS: 0.0516
%SA: 0.0624. }\label{tab:RNN:RMSE}
%\end{table}

%
%\begin{table}[ht]
%\centering\small\renewcommand\arraystretch{1.25}
%\begin{tabular}{c|cccccc}
%  \hline
%Method & 1 hour & 2 hours & 3 hours & 6 hours & 12 hours & 24 hours \\ 
%  \hline
%RNNC & 32.5610 & 32.9776 & 33.1809 & 33.8470 & 32.8989 & 31.7415 \\ 
%  GAMLSS & 33.5579 & 34.5999 & 39.7815 & 46.3045 & 71.7834 & 305.0956 \\ 
%  RNNST & 33.2465 & 33.5892 & 33.7738 & 33.8191 & 33.7791 & 34.0819 \\ 
%  RNNSN & 36.6275 & 36.4510 & 36.3765 & 35.8254 & 37.7442 & 36.9532 \\ 
%  RNN & 34.1640 & 34.4068 & 34.5347 & 34.6406 & 34.7903 & 35.0608 \\  
%   \hline
%\end{tabular}
% \caption{System weighted joint score computed from the simulated ahead forecast values for $\alpha=0.975$.
% 	Results from all three models are shown, these are RNNC, GAMLSS, RNNSN, RNN. Lower values correspond to higher predictive accuracy. The system weights are: NSW: 0.3687
%VIC: 0.2355
%QLD: 0.2818
%TAS: 0.0516
%SA: 0.0624. }\label{tab:RNN:JS}
%\end{table}


%\begin{table}[ht]
%\centering\small\renewcommand\arraystretch{1.25}
%\begin{tabular}{c|cccccc}
%  \hline
%Method & 1 hour & 2 hours & 3 hours & 6 hours & 12 hours & 24 hours \\ 
%  \hline
%RNNC & 0.0089 & 0.0092 & 0.0093 & 0.0095 & 0.0091 & 0.0089 \\ 
%  GAMLSS & 0.0093 & 0.0113 & 0.0118 & 0.0141 & 0.0196 & 0.0317 \\ 
%  RNNST & 0.0086 & 0.0087 & 0.0088 & 0.0088 & 0.0088 & 0.0089 \\ 
%  RNNSN & 0.0105 & 0.0107 & 0.0113 & 0.0109 & 0.0112 & 0.0113 \\ 
%  RNN & 0.0140 & 0.0141 & 0.0142 & 0.0146 & 0.0148 & 0.0155 \\ 
%   \hline
%\end{tabular}
% \caption{System weighted mean quantile score computed from the simulated ahead forecast values.
% 	Results from all three models are shown, these are RNNC, GAMLSS, RNNSN, RNN. Lower values correspond to higher predictive accuracy. The system weights are: NSW: 0.3687
%VIC: 0.2355
%QLD: 0.2818
%TAS: 0.0516
%SA: 0.0624. }\label{tab:RNN:QS}
%\end{table}

\begin{table}[ht]
\begin{center}
\centering\small\renewcommand\arraystretch{1.25}
 \caption{Coverage of 95\% prediction intervals during the 
	evaluation period.}\label{tab:RNN:covs}
\begin{tabular}{lccccccc}
  \hline
		&\multicolumn{7}{c}{Hours Ahead in the Forecast Horizon}\\ \cline{2-8}
		Model & 0.5 hour & 1 hour & 2 hours & 3 hours & 6 hours & 12 hours & 24 hours  \\ \hline
GAMLSS & 0.9078 & 0.8148 & 0.7278 & 0.6928 & 0.6476 & 0.5838 & 0.5208 \\ 
  RNN & 0.8715 & 0.8609 & 0.7906 & 0.7173 & 0.6336 & 0.5698 & 0.6124 \\ 
  RNNSN & 0.8496 & 0.8386 & 0.8354 & 0.8187 & 0.8123 & 0.7998 & 0.7759 \\ 
  RNNST & 0.8550 & 0.8424 & 0.8353 & 0.8216 & 0.8171 & 0.7955 & 0.7667 \\ 
  \emph{RNNC} & \emph{0.9279} & \emph{0.9012} & \emph{0.8791} & \emph{0.8741} & \emph{0.8620} & \emph{0.8594} & \emph{0.8706} \\ 
   \hline
\end{tabular}
\end{center}
  Results are reported
 	for the four deep time series models, plus
 	GAMLSS, at different points in time in the 24 hour forecast horizon.
 	Values closer to 0.95 indicate improved calibration of the probabilistic forecasts.
\end{table}

\begin{table}[htb]
	\begin{center}
\centering\small\renewcommand\arraystretch{1.25}
 \caption{NSW price forecast accuracy when
 	including demand forecast information.} \label{tab:foredemand}
\begin{tabular}{lllllllll}
  \hline\hline
Model &  MAE & RMSE & CRPS & &JS &QS95 & QS05 & C95 \\ 
  \hline
&   \multicolumn{3}{l}{Point and Density Accuracy} &  &\multicolumn{3}{l}{Tail Accuracy} & \\ \cline{2-4} \cline{6-8}
%  &\multicolumn{6}{l}{Without Demand Forecasts as Features}\\ \cline{2-8}
\textit{RNNC+D} & \textit{0.0192 } &  \textit{0.0314}  &  \textit{0.0146} & & \textit{30.6902}  &  \textit{0.0045}   & \textit{0.0025} & 82.6\% \\
RNNC & 0.0188$^{\mbox{\tiny{+++}}}$   & 0.0311$^{\mbox{\tiny{+++}}}$ &  0.0144$^{\mbox{\tiny{+++}}}$ &&  31.0350$^{**}$  &  0.0048$^{***}$    & 0.0023 & 84.5\% \\   
%  &\multicolumn{6}{l}{Including Demand Forecasts as Features}\\ \cline{2-8}
%  RNNCcov & 0.0115 & 0.0313 & 0.0143 & 30.4646 & 0.0069 & \textbf{0.8390} \\ 
%  RNNSTcov   & 0.0147 & 0.0316 & 0.0160 & 31.8385 & 0.0078 & 0.8128 \\ 
 RNNST &0.0250$^{***}$    &0.0401    &0.0221$^{***}$ &  &39.4411$^{***}$    &0.0121$^{***}$    &0.0049$^{***}$ & 46.2 \%\\
  RNNST+D & 0.0256$^{***}$ &   0.0395  &  0.0222$^{***}$ && 39.6431$^{***}$   & 0.0123$^{***}$  &  0.0046$^{***}$ & 53.9\% \\ 
   \hline\hline
\end{tabular}
\end{center}
 Accuracy of 24 hour ahead NSW (logarithmic) price forecasts during the evaluation period. Models that include 24 hour ahead demand forecast information as features are labelled as ``+D''. The metrics are described in the text, and
include the joint score (JS) at $\alpha=0.975$, quantile score (QS) at $\alpha=0.95,0.05$, and the empirical coverage of the 95\% prediction intervals (C95). %The stars ``*'', ``**'' ,``***'' at RNNC+D indicate significantly better metrics for RNNC+D than for RNNC at the $1,5,10\%$ levels using a two-sided Diebold-Marino (DM) test statistic. Similarly for RNNST+D and RNNST+D.
Results of a two-sided Diebold-Mariano test of the equality of the mean error of the RNNC+D with the other methods are reported. Rejection of the null hypothesis of equal means at the 10\%, 5\% and 1\% levels are denoted by ``*'', ``**'' and ``***'' if favorable to the RNNC+D model, or by ``${\mbox{\tiny{+}}}$'', ``${\mbox{\tiny{++}}}$'' and ``${\mbox{\tiny{+++}}}$'' if unfavorable.
\end{table}



%Results of a two-sided Diebold-Mariano test of the equality of the mean error of the RNNC with each of the other models are reported. Rejection of the null hypothesis of equal means at the 10\%, 5\% and 1\% levels are denoted by ``*'', ``**'' and ``***'' if favorable to the RNNC model, or by ``${\mbox{\tiny{+}}}$'', %``${\mbox{\tiny{++}}}$'' and
%		``${\mbox{\tiny{+++}}}$'' if unfavorable.

